Mask the Unknown: Assessing Different Strategies to Handle Weak Annotations in the MICCAI2023 Mediastinal Lymph Node Quantification Challenge

Pathological lymph node delineation is crucial in cancer diagnosis, progression assessment, and treatment planning. The MICCAI 2023 Lymph Node Quantification Challenge published the first public dataset for pathological lymph node segmentation in the mediastinum. As lymph node annotations are expensive, the challenge was formed as a weakly supervised learning task, where only a subset of all lymph nodes in the training set have been annotated. For the challenge submission, multiple methods for training on these weakly supervised data were explored, including noisy label training, loss masking of unlabeled data, and an approach that integrated the TotalSegmentator toolbox as a form of pseudo labeling in order to reduce the number of unknown voxels. Furthermore, multiple public TCIA datasets were incorporated into the training to improve the performance of the deep learning model. Our submitted model achieved a Dice score of 0.628 and an average symmetric surface distance of 5.8~mm on the challenge test set. With our submitted model, we accomplished third rank in the MICCAI2023 LNQ challenge. A finding of our analysis was that the integration of all visible, including non-pathological, lymph nodes improved the overall segmentation performance on pathological lymph nodes of the test set. Furthermore, segmentation models trained only on clinically enlarged lymph nodes, as given in the challenge scenario, could not generalize to smaller pathological lymph nodes. The code and model for the challenge submission are available at \url{https://gitlab.lrz.de/compai/MediastinalLymphNodeSegmentation}.

==> Makefile <==
CC = latexmk
CFLAGS = -use-make -pdflatex -silent -time

.PHONY: all clean FORCE

MAINDIR = ..

PDFS = $(MAINDIR)/melba-sample-accepted-special-issue.pdf \
	$(MAINDIR)/melba-sample-accepted.pdf \
	$(MAINDIR)/melba-sample-in-submission.pdf \
	$(MAINDIR)/melba-sample-arxiv-submission.pdf \
	$(MAINDIR)/melba-sample.pdf


all: $(PDFS)

melba.sty: $(MAINDIR)/melba.sty
	cp $< $@

sample.bib: $(MAINDIR)/sample.bib
	cp $< $@

melba-sample-%.tex: $(MAINDIR)/melba-sample.tex melba-sample-%.patch
	patch $^ -o $@

$(MAINDIR)/melba-sample-%.pdf: melba-sample-%.tex melba.sty sample.bib FORCE
	$(CC) $(CFLAGS) $<
	cp $(@F) $@

$(MAINDIR)/melba-sample.pdf: $(MAINDIR)/melba-sample.tex melba.sty FORCE
	$(CC) $(CFLAGS) $<
	cp $(@F) $@


clean:
	rm -f *.aux *.bbl *.blg *.log *.fls *.fdb_latexmk
	rm -f melba-sample-*.tex
	rm -f *.out
	rm -f *.tex melba.sty sample.bib

FORCE:

